On Optimal Neighbor Discovery

Mobile devices apply neighbor discovery (ND) protocols to wirelessly initiate a first contact within the shortest possible amount of time and with minimal energy consumption. For this purpose, over the last decade, a vast number of ND protocols have been proposed, which have progressively reduced the relation between the time within which discovery is guaranteed and the energy consumption. In spite of the simplicity of the problem statement, even after more than 10 years of research on this specific topic, new solutions are still proposed even today. Despite the large number of known ND protocols, given an energy budget, what is the best achievable latency still remains unclear. This paper addresses this question and for the first time presents safe and tight, duty-cycle-dependent bounds on the worst-case discovery latency that no ND protocol can beat. Surprisingly, several existing protocols are indeed optimal, which has not been known until now. We conclude that there is no further potential to improve the relation between latency and duty-cycle, but future ND protocols can improve their robustness against beacon collisions.

==> sections/evaluation.tex <==
\vspace*{-0.5em}
\section{Evaluation}
\label{sec:evaluation}
In this section, we numerically evaluate the bounds from Section \ref{sec:bounds} to obtain insights on the performance of optimal \ac{ND} protocols.
\subsection{Asymmetric Protocols}
\begin{figure}[tb]
	\centering
	\includegraphics[width=\imgWidth]{images/assymBoundSurfPlot_product.png}
	\caption{Product of the worst-case bound and the sum of duty-cycles $\eta_E + \eta_F$ of two devices.}
	\label{fig:asymBoundSurfPlot_product} 
\end{figure}

Asymmetric \ac{ND} protocols are of high practical relevance, since they allow multiple devices with different energy consumptions or different power budgets to operate on different duty-cycles.
% Especially, protocols that guarantee bounded discovery even if the duty-cycle of the opposite device is unknown are of tremendous practical use, since every device may adjust its duty-cycle on the fly, based on e.g., its battery level or the amount of harvested energy. 
We therefore in the following study the energy overhead of asymmetry. As the main metric for energy consumption, we consider the joint duty-cycle $\eta_E + \eta_F$ of two devices \textit{E} and \textit{F}. 
Figure \ref{fig:asymBoundSurfPlot_product} depicts the product of the joint duty-cycle and the worst-case latency $L$, as given by Theorem \ref{thm:asymBound}. In addition, the bound for $\eta_E = \eta_F$ (i.e., for symmetric discovery) is shown.
As can be seen, $L \cdot (\eta_E + \eta_F)$ only depends on the sum $\eta_E + \eta_F$ and not on the actual degree of asymmetry $|\eta_E - \eta_F|$. In other words, there is no ``cost'' for asymmetry, since asymmetric protocols can achieve the same worst-case latency as symmetric ones for a given sum of duty-cycles.

\subsection{Constrained Collision Probability}
\label{sec:collision_constraint_eval}
\begin{figure}[bt]
	\centering
	\includegraphics[width=\imgWidth]{images/chanUtilConstraintPlot.png}
	\caption{Bounds on $\mathbf{L}$ when limiting the collision rate to $\mathbf{\SI{1}{\percent}}$ for different numbers of transmitters $\mathbf{S}$.}
	\label{fig:chanUtilConstraintPlot} 
\end{figure}
In this section, we study how constraints on the collision probability impact the worst-case performance.
%Let us consider a number of $S-1$ senders, of which each causes a channel utilization of $\beta$. Under the assumption of independent beacon transmissions by multiple senders, the first beacon of an additional sender that starts transmitting (or comes into range) at any random point in time will face a collision probability of \cite{abramson:70}:
%\begin{equation}
%\label{eq:abramsonCollisions}
%P_{c} = 1-e^{-2 (S - 1) \cdot \beta}
%\end{equation}
%\nomenclature{$S$}{Number of transmitting devices}
%\nomenclature{$P_c$}{Collision probability}
%Note that once a beacon has collided with a beacon from another device, the repetitiveness of the infinite %beacon sequence implies that the fraction of later beacons colliding with the same node is predefined. 
%Nevertheless, since all offsets between the two sequences occur with the same probability, the collision probability of any individual beacon in the beacon sequence is given by Equation~\ref{eq:abramsonCollisions}. We can therefore express the maximum channel utilization $\beta_m$ by $P_c$ and apply Theorem~\ref{thm:boundSymChannelConstraint} to obtain a latency bound for any given maximum collision probability $P_c$.
Figure~\ref{fig:chanUtilConstraintPlot} depicts such latency bounds for a maximum collision probability $P_c$ of $\SI{1}{\percent}$ and different numbers of interfering senders $S$. As can be seen, for small duty-cycles, the latency bound remains unaffected by this constraint, since the collision probability is anyway below the threshold $P_c$. Starting from the duty-cycles marked with circles, the bound gets deteriorated by up to two orders of magnitude. Therefore, protocols that scale towards larger, busy networks need to sacrifice some of their performance for small networks.

==> sections/glossary.tex <==
\newacronym{MANET}{MANET}{mobile ad-hoc network}
\newacronym{ND}{ND}{neighbor discovery}
\newacronym{BLE}{BLE}{Bluetooth Low Energy}
\newacronym{PI}{PI}{periodic interval}
